On Implicit Regularization in $\beta$-VAEs

While the impact of variational inference (VI) on posterior inference in a fixed generative model is well-characterized, its role in regularizing a learned generative model when used in variational autoencoders (VAEs) is poorly understood. We study the regularizing effects of variational distributions on learning in generative models from two perspectives. First, we analyze the role that the choice of variational family plays in imparting uniqueness to the learned model by restricting the set of optimal generative models. Second, we study the regularization effect of the variational family on the local geometry of the decoding model. This analysis uncovers the regularizer implicit in the $\beta$-VAE objective, and leads to an approximation consisting of a deterministic autoencoding objective plus analytic regularizers that depend on the Hessian or Jacobian of the decoding model, unifying VAEs with recent heuristics proposed for training regularized autoencoders. We empirically verify these findings, observing that the proposed deterministic objective exhibits similar behavior to the $\beta$-VAE in terms of objective value and sample quality.

==> dump.tex <==
\begin{figure*}[t]
\centering
\subfigure[$\beta=0.4,d=12,b=3$]{\label{fig:blksz3_a}\includegraphics[width=0.17\textwidth]{figures/jjt_plots_blk3/enccov-inv 20-beta=0.4,lr=0.001,block_diag_size=3,latent_dim=12,layer_width=64.png} 
\includegraphics[width=0.17\textwidth]{figures/jjt_plots_blk3/JJT 20-beta=0.4,lr=0.001,block_diag_size=3,latent_dim=12,layer_width=64.png}}~
\subfigure[$\beta=0.6,d=8,b=3$]{\label{fig:blksz3_b}\includegraphics[width=0.17\textwidth]{figures/jjt_plots_blk3/enccov_inv 34-beta=0.6,lr=0.001,block_diag_size=3,latent_dim=8,layer_width=64.png}
\includegraphics[width=0.17\textwidth]{figures/jjt_plots_blk3/JJT 34-beta=0.6,lr=0.001,block_diag_size=3,latent_dim=8,layer_width=64.png}}~
\subfigure[$\beta=0.8,d=20,b=3$]{\label{fig:blksz3_c}\includegraphics[width=0.17\textwidth]{figures/jjt_plots_blk3/enccov_inv 48-beta=0.8,lr=0.001,block_diag_size=3,latent_dim=20,layer_width=64.png}
\includegraphics[width=0.17\textwidth]{figures/jjt_plots_blk3/JJT 48-beta=0.8,lr=0.001,block_diag_size=3,latent_dim=20,layer_width=64.png}}
\caption{Posterior precision matrices $\Sigma_{z|x}^{-1}$ (left) and the corresponding $J_g(h(x))^\top J_g(h(x))$ (right) for different values of $\beta$ and latent dimensionality $d$. Block sizes $b$ for the posterior covariance was taken to be $3$ for each setting.}
\label{fig:blksz3}
\end{figure*}


\begin{table*}[t]
\caption{CelebA samples using the standard normal prior for $\beta$-VAE and Gaussian-RAE (Eq.~\eqref{eq:elbo_gauss_obs}) for different values of $\beta$. Samples from models trained using the GRAE objective have similar smoothness/blurriness as samples from $\beta$-VAE models for a wide range of $\beta$.}
\vspace{3mm}
\centering
\begin{tabular}{lcccc}
& $\beta=0.02$ & $\beta=0.04$ & $\beta=0.06$ & $\beta=0.08$  \\
\rotatebox[origin=c]{90}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~{\bf VAE} Samples}\hspace{-4mm} & \includegraphics[width=0.23\textwidth]{figures/celeba_vae/4-beta=0.02,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/6-beta=0.04,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/8-beta=0.06,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/10-beta=0.08,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png} \vspace{-25mm}\\
\rotatebox[origin=c]{90}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~{\bf GRAE} Samples}\hspace{-4mm} & \includegraphics[width=0.23\textwidth]{figures/celeba_rae/7-lr=0.001,beta=0.02,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/11-lr=0.001,beta=0.04,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/15-lr=0.001,beta=0.06,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/19-lr=0.001,beta=0.08,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png} \vspace{-25mm}\\
& $\beta=0.1$ & $\beta=0.2$ & $\beta=0.4$ & $\beta=0.8$  \\
\rotatebox[origin=c]{90}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~{\bf VAE} Samples}\hspace{-4mm} & \includegraphics[width=0.23\textwidth]{figures/celeba_vae/12-beta=0.1,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/13-beta=0.2,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/15-beta=0.4,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/19-beta=0.8,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png} \vspace{-25mm}\\
\rotatebox[origin=c]{90}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~{\bf GRAE} Samples}\hspace{-4mm} & \includegraphics[width=0.23\textwidth]{figures/celeba_rae/23-lr=0.001,beta=0.1,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/25-lr=0.001,beta=0.2,lambda_orth=0.01__it25999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/29-lr=0.001,beta=0.4,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/37-lr=0.001,beta=0.8,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png} \vspace{-20mm}
\end{tabular}
\label{tab:celebasamples_betasweep}
\end{table*}

\begin{table*}[t]
\caption{CelebA samples using the standard normal prior for $\beta$-VAE and Gaussian-RAE) for different values of $\beta$. Samples from models trained using the GRAE objective have similar smoothness/blurriness as samples from $\beta$-VAE models for a wide range of $\beta$.}
\centering
\begin{tabular}{lcccc}
& $\beta=0.02$ & $\beta=0.04$ & $\beta=0.06$ & $\beta=0.08$  \\
\rotatebox[origin=c]{90}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~{\bf VAE} Samples}\hspace{-4mm} & \includegraphics[width=0.23\textwidth]{figures/celeba_vae/4-beta=0.02,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/6-beta=0.04,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/8-beta=0.06,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/10-beta=0.08,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png} \vspace{-25mm}\\
\rotatebox[origin=c]{90}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~{\bf GRAE} Samples}\hspace{-4mm} & \includegraphics[width=0.23\textwidth]{figures/celeba_rae/7-lr=0.001,beta=0.02,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/11-lr=0.001,beta=0.04,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/15-lr=0.001,beta=0.06,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/19-lr=0.001,beta=0.08,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png} \vspace{-25mm}\\
& $\beta=0.1$ & $\beta=0.2$ & $\beta=0.4$ & $\beta=0.8$  \\
\rotatebox[origin=c]{90}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~{\bf VAE} Samples}\hspace{-4mm} & \includegraphics[width=0.23\textwidth]{figures/celeba_vae/12-beta=0.1,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/13-beta=0.2,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/15-beta=0.4,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_vae/19-beta=0.8,lr=0.001,latent_dim=128__it49999_0_size_4x4_decoder_samples_stdnormal.png} \vspace{-25mm}\\
\rotatebox[origin=c]{90}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~{\bf GRAE} Samples}\hspace{-4mm} & \includegraphics[width=0.23\textwidth]{figures/celeba_rae/23-lr=0.001,beta=0.1,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/25-lr=0.001,beta=0.2,lambda_orth=0.01__it25999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/29-lr=0.001,beta=0.4,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png}\hspace{-2mm} &
\includegraphics[width=0.23\textwidth]{figures/celeba_rae/37-lr=0.001,beta=0.8,lambda_orth=0.01__it39999_0_size_4x4_decoder_samples_stdnormal.png} \vspace{-20mm}
\end{tabular}
\label{tab:celebasamples_betasweep_appendix}
\end{table*}

